The Gap Between Greedy Algorithm and Minimum Multiplicative Spanner

The greedy algorithm adapted from Kruskal's algorithm is an efficient and folklore way to produce a $k$-spanner with girth at least $k+2$. The greedy algorithm has shown to be `existentially optimal', while it's not `universally optimal' for any constant $k$. Here, `universal optimality' means an algorithm can produce the smallest $k$-spanner $H$ given any $n$-vertex input graph $G$. However, how well the greedy algorithm works compared to `universal optimality' is still unclear for superconstant $k:=k(n)$. In this paper, we aim to give a new and fine-grained analysis of this problem in undirected unweighted graph setting. Specifically, we show some bounds on this problem including the following two (1) On the negative side, when $k<\frac{1}{3}n-O(1)$, the greedy algorithm is not `universally optimal'. (2) On the positive side, when $k>\frac{2}{3}n+O(1)$, the greedy algorithm is `universally optimal'. We also introduce an appropriate notion for `approximately universal optimality'. An algorithm is $(\alpha,\beta)$-universally optimal iff given any $n$-vertex input graph $G$, it can produce a $k$-spanner $H$ of $G$ with size $|H|\leq n+\alpha(|H^*|-n)+\beta$, where $H^*$ is the smallest $k$-spanner of $G$. We show the following positive bounds. (1) When $k>\frac{4}{7}n+O(1)$, the greedy algorithm is $(2,O(1))$-universally optimal. (2) When $k>\frac{12}{23}n+O(1)$, the greedy algorithm is $(18,O(1))$-universally optimal. (3) When $k>\frac{1}{2}n+O(1)$, the greedy algorithm is $(32,O(1))$-universally optimal. All our proofs are constructive building on new structural analysis on spanners. We give some ideas about how to break small cycles in a spanner to increase the girth. These ideas may help us to understand the relation between girth and spanners.

==> abstract.tex <==
\begin{abstract}
	\hanlin{Goals of this paper:} (1) Prove that a non-trivial algorithm $\ckt\SatPair$ implies both avoidance algorithms in $\FP^\NP$ and hard partial truth table in $\FP^\NP$; (2) finding a better algorithm for $\ACC^0\SatPair$ and maybe also $\NC^0\SatPair$ with better parameters; (3) extend the framework of RSW22 to strong average-case lbs using an error correcting code with linear sum decoders.
	
	TODO: More goals?
\end{abstract}

\begin{center}
	\Large \bf TODO List
\end{center}
\begin{compactitem}
	\item \sout{Note: use ``sout'' comment to strikeout anything that's already done.}
	\item Propose a title
	\item Write section 1.2 (our results).
	\item Write a related work section
	\item Write a technical overview section
	\item decide zero or one index
	\item change ``fanin'' to ``fan-in''
	\item decide US or UK English
	\item change $\Pi_d$ to $\Prod_d$
\end{compactitem}

\begin{center}
	\Large \bf Status of each section
\end{center}

Note: emphasize the current status. Just ensure that everything pass ``preliminary'' review before the deadline; when we post a final version everything should pass serious review. Let's also add comments under these sections.

\begin{itemize}
	\item abstract (\emph{under construction}, need review, passed preliminary review, passed serious review)
	\item Section 1 (\emph{under construction}, need review, passed preliminary review, passed serious review)
	\item Section 2 (under construction, need review, \emph{passed preliminary review}, passed serious review)
	\begin{compactitem}
		\item \hanlin{I went through everything in sec 2. In case that more will be added in sec 2: what I went through was sec 2.1 (circuit classes), 2.2 (ECC), 2.3 (hierarchy with refuter), 2.4 (linear sum), 2.5 (PCPP), 2.6 (alg and reduction), 2.7 (NC0 Satpair from AND satpair). All of them are good, except for the notes that aren't removed yet.}
	\end{compactitem}
	\item Section 3 (under construction, \emph{need review}, passed preliminary review, passed serious review)
	\begin{compactitem}
	\item \jiatu{I'm making a pass on this!}
	\item \yeyuan{remote point reviewed, comments in sec3.2}
	\end{compactitem}
	\item Section 4 (\emph{under construction}, need review, passed preliminary review, passed serious review)
	\item Section 5 (\emph{under construction}, need review, passed preliminary review, passed serious review)
	\item Section 6 (\emph{under construction}, need review, passed preliminary review, passed serious review)
	\item Section 7 (under construction, need review, \emph{passed preliminary review}, passed serious review)
	\item Section 8 (under construction, need review, \emph{passed preliminary review}, passed serious review)
	\item bibliography (under construction, \emph{need review}, passed preliminary review, passed serious review)
	\item Section A (under construction, need review, \emph{passed preliminary review}, passed serious review)
	\begin{compactitem}
		\item \hanlin{I went through most of this section, it seems good. I left one comment in it where some $\ell^2$ bound can be improved to $\ell$, but it doesn't affect the overall complexity. I also still need to check the time bounds.}
	\end{compactitem}
	\item Section B (under construction, \emph{need review}, passed preliminary review, passed serious review)
	\begin{compactitem}
		\item \hanlin{If we don't have enough time then don't need to review this. It's not urgent and I'm quite confident that this works out. :)}
	\end{compactitem}	
\end{itemize}

\hanlin{Note: I'm using the ``condensed'' version of DBLP bib entries}

